Search-Guided, Lightly-supervised Training of Structured Prediction Energy Networks

In structured output prediction tasks, labeling ground-truth training output is often expensive. However, for many tasks, even when the true output is unknown, we can evaluate predictions using a scalar reward function, which may be easily assembled from human knowledge or non-differentiable pipelines. But searching through the entire output space to find the best output with respect to this reward function is typically intractable. In this paper, we instead use efficient truncated randomized search in this reward function to train structured prediction energy networks (SPENs), which provide efficient test-time inference using gradient-based search on a smooth, learned representation of the score landscape, and have previously yielded state-of-the-art results in structured prediction. In particular, this truncated randomized search in the reward function yields previously unknown local improvements, providing effective supervision to SPENs, avoiding their traditional need for labeled training data.

==> plot.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(110.0,82.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,82){\makebox(0,0)[r]{$0$}}
\put(1419.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,179.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,179.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,179){\makebox(0,0)[r]{$0.1$}}
\put(1419.0,179.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,276.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,276.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,276){\makebox(0,0)[r]{$0.2$}}
\put(1419.0,276.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,373.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,373.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,373){\makebox(0,0)[r]{$0.3$}}
\put(1419.0,373.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,471.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,471.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,471){\makebox(0,0)[r]{$0.4$}}
\put(1419.0,471.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,568.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,568.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,568){\makebox(0,0)[r]{$0.5$}}
\put(1419.0,568.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,665.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,665.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,665){\makebox(0,0)[r]{$0.6$}}
\put(1419.0,665.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,762.0){\rule[-0.200pt]{204.524pt}{0.400pt}}
\put(1419.0,762.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,762.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,762){\makebox(0,0)[r]{$0.7$}}
\put(1419.0,762.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,859.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(110.0,859.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90,859){\makebox(0,0)[r]{$0.8$}}
\put(1419.0,859.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(110.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(110,41){\makebox(0,0){$0$}}
\put(110.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(243.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(243.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(243,41){\makebox(0,0){$10$}}
\put(243.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(376.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(376.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(376,41){\makebox(0,0){$20$}}
\put(376.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(509.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(509.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(509,41){\makebox(0,0){$30$}}
\put(509.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(642.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(642.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(642,41){\makebox(0,0){$40$}}
\put(642.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(775.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(775.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(775,41){\makebox(0,0){$50$}}
\put(775.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(907.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(907.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(907,41){\makebox(0,0){$60$}}
\put(907.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1040.0,82.0){\rule[-0.200pt]{0.400pt}{162.607pt}}
\put(1040.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1040.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1040,41){\makebox(0,0){$70$}}
\put(1040.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1173.0,82.0){\rule[-0.200pt]{0.400pt}{162.607pt}}
\put(1173.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1173.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1173,41){\makebox(0,0){$80$}}
\put(1173.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1306.0,82.0){\rule[-0.200pt]{0.400pt}{162.607pt}}
\put(1306.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1306.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1306,41){\makebox(0,0){$90$}}
\put(1306.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1439,41){\makebox(0,0){$100$}}
\put(1439.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(110.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(110.0,82.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(110.0,859.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(1279,818){\makebox(0,0)[r]{$alpha=0.01$}}
\put(110,92){\makebox(0,0){$+$}}
\put(123,97){\makebox(0,0){$+$}}
\put(137,146){\makebox(0,0){$+$}}
\put(150,169){\makebox(0,0){$+$}}
\put(163,192){\makebox(0,0){$+$}}
\put(176,227){\makebox(0,0){$+$}}
\put(190,248){\makebox(0,0){$+$}}
\put(203,260){\makebox(0,0){$+$}}
\put(216,279){\makebox(0,0){$+$}}
\put(230,300){\makebox(0,0){$+$}}
\put(243,311){\makebox(0,0){$+$}}
\put(256,329){\makebox(0,0){$+$}}
\put(269,344){\makebox(0,0){$+$}}
\put(283,365){\makebox(0,0){$+$}}
\put(296,378){\makebox(0,0){$+$}}
\put(309,400){\makebox(0,0){$+$}}
\put(323,420){\makebox(0,0){$+$}}
\put(336,430){\makebox(0,0){$+$}}
\put(349,448){\makebox(0,0){$+$}}
\put(363,461){\makebox(0,0){$+$}}
\put(376,471){\makebox(0,0){$+$}}
\put(389,495){\makebox(0,0){$+$}}
\put(402,512){\makebox(0,0){$+$}}
\put(416,526){\makebox(0,0){$+$}}
\put(429,534){\makebox(0,0){$+$}}
\put(442,546){\makebox(0,0){$+$}}
\put(456,551){\makebox(0,0){$+$}}
\put(469,565){\makebox(0,0){$+$}}
\put(482,567){\makebox(0,0){$+$}}
\put(495,576){\makebox(0,0){$+$}}
\put(509,585){\makebox(0,0){$+$}}
\put(522,597){\makebox(0,0){$+$}}
\put(535,598){\makebox(0,0){$+$}}
\put(549,598){\makebox(0,0){$+$}}
\put(562,611){\makebox(0,0){$+$}}
\put(575,612){\makebox(0,0){$+$}}
\put(588,630){\makebox(0,0){$+$}}
\put(602,642){\makebox(0,0){$+$}}
\put(615,653){\makebox(0,0){$+$}}
\put(628,656){\makebox(0,0){$+$}}
\put(642,655){\makebox(0,0){$+$}}
\put(655,663){\makebox(0,0){$+$}}
\put(668,672){\makebox(0,0){$+$}}
\put(681,679){\makebox(0,0){$+$}}
\put(695,676){\makebox(0,0){$+$}}
\put(708,691){\makebox(0,0){$+$}}
\put(721,697){\makebox(0,0){$+$}}
\put(735,690){\makebox(0,0){$+$}}
\put(748,695){\makebox(0,0){$+$}}
\put(761,704){\makebox(0,0){$+$}}
\put(775,705){\makebox(0,0){$+$}}
\put(788,719){\makebox(0,0){$+$}}
\put(801,717){\makebox(0,0){$+$}}
\put(814,723){\makebox(0,0){$+$}}
\put(828,726){\makebox(0,0){$+$}}
\put(841,726){\makebox(0,0){$+$}}
\put(854,735){\makebox(0,0){$+$}}
\put(868,739){\makebox(0,0){$+$}}
\put(881,742){\makebox(0,0){$+$}}
\put(894,743){\makebox(0,0){$+$}}
\put(907,747){\makebox(0,0){$+$}}
\put(921,743){\makebox(0,0){$+$}}
\put(934,733){\makebox(0,0){$+$}}
\put(947,744){\makebox(0,0){$+$}}
\put(961,751){\makebox(0,0){$+$}}
\put(974,752){\makebox(0,0){$+$}}
\put(987,746){\makebox(0,0){$+$}}
\put(1000,756){\makebox(0,0){$+$}}
\put(1014,758){\makebox(0,0){$+$}}
\put(1027,767){\makebox(0,0){$+$}}
\put(1040,770){\makebox(0,0){$+$}}
\put(1054,768){\makebox(0,0){$+$}}
\put(1067,762){\makebox(0,0){$+$}}
\put(1080,764){\makebox(0,0){$+$}}
\put(1093,771){\makebox(0,0){$+$}}
\put(1107,769){\makebox(0,0){$+$}}
\put(1120,779){\makebox(0,0){$+$}}
\put(1133,785){\makebox(0,0){$+$}}
\put(1147,798){\makebox(0,0){$+$}}
\put(1160,803){\makebox(0,0){$+$}}
\put(1173,799){\makebox(0,0){$+$}}
\put(1186,797){\makebox(0,0){$+$}}
\put(1200,791){\makebox(0,0){$+$}}
\put(1213,790){\makebox(0,0){$+$}}
\put(1226,798){\makebox(0,0){$+$}}
\put(1240,801){\makebox(0,0){$+$}}
\put(1253,805){\makebox(0,0){$+$}}
\put(1266,796){\makebox(0,0){$+$}}
\put(1280,792){\makebox(0,0){$+$}}
\put(1293,797){\makebox(0,0){$+$}}
\put(1306,804){\makebox(0,0){$+$}}
\put(1319,810){\makebox(0,0){$+$}}
\put(1333,807){\makebox(0,0){$+$}}
\put(1346,802){\makebox(0,0){$+$}}
\put(1359,809){\makebox(0,0){$+$}}
\put(1373,811){\makebox(0,0){$+$}}
\put(1386,801){\makebox(0,0){$+$}}
\put(1399,804){\makebox(0,0){$+$}}
\put(1412,809){\makebox(0,0){$+$}}
\put(1426,813){\makebox(0,0){$+$}}
\put(1349,818){\makebox(0,0){$+$}}
\put(1279,777){\makebox(0,0)[r]{"bib2" using 1:3}}
\put(110,117){\makebox(0,0){$\times$}}
\put(123,119){\makebox(0,0){$\times$}}
\put(137,120){\makebox(0,0){$\times$}}
\put(150,119){\makebox(0,0){$\times$}}
\put(163,119){\makebox(0,0){$\times$}}
\put(176,121){\makebox(0,0){$\times$}}
\put(190,124){\makebox(0,0){$\times$}}
\put(203,124){\makebox(0,0){$\times$}}
\put(216,126){\makebox(0,0){$\times$}}
\put(230,128){\makebox(0,0){$\times$}}
\put(243,129){\makebox(0,0){$\times$}}
\put(256,131){\makebox(0,0){$\times$}}
\put(269,133){\makebox(0,0){$\times$}}
\put(283,136){\makebox(0,0){$\times$}}
\put(296,138){\makebox(0,0){$\times$}}
\put(309,142){\makebox(0,0){$\times$}}
\put(323,144){\makebox(0,0){$\times$}}
\put(336,149){\makebox(0,0){$\times$}}
\put(349,161){\makebox(0,0){$\times$}}
\put(363,179){\makebox(0,0){$\times$}}
\put(376,221){\makebox(0,0){$\times$}}
\put(389,249){\makebox(0,0){$\times$}}
\put(402,273){\makebox(0,0){$\times$}}
\put(416,299){\makebox(0,0){$\times$}}
\put(429,322){\makebox(0,0){$\times$}}
\put(442,347){\makebox(0,0){$\times$}}
\put(456,375){\makebox(0,0){$\times$}}
\put(469,423){\makebox(0,0){$\times$}}
\put(482,465){\makebox(0,0){$\times$}}
\put(495,491){\makebox(0,0){$\times$}}
\put(509,508){\makebox(0,0){$\times$}}
\put(522,519){\makebox(0,0){$\times$}}
\put(535,529){\makebox(0,0){$\times$}}
\put(549,543){\makebox(0,0){$\times$}}
\put(562,540){\makebox(0,0){$\times$}}
\put(575,565){\makebox(0,0){$\times$}}
\put(588,579){\makebox(0,0){$\times$}}
\put(602,579){\makebox(0,0){$\times$}}
\put(615,587){\makebox(0,0){$\times$}}
\put(628,594){\makebox(0,0){$\times$}}
\put(642,604){\makebox(0,0){$\times$}}
\put(655,612){\makebox(0,0){$\times$}}
\put(668,621){\makebox(0,0){$\times$}}
\put(681,625){\makebox(0,0){$\times$}}
\put(695,628){\makebox(0,0){$\times$}}
\put(708,630){\makebox(0,0){$\times$}}
\put(721,651){\makebox(0,0){$\times$}}
\put(735,657){\makebox(0,0){$\times$}}
\put(748,655){\makebox(0,0){$\times$}}
\put(761,663){\makebox(0,0){$\times$}}
\put(775,672){\makebox(0,0){$\times$}}
\put(788,670){\makebox(0,0){$\times$}}
\put(801,676){\makebox(0,0){$\times$}}
\put(814,684){\makebox(0,0){$\times$}}
\put(828,690){\makebox(0,0){$\times$}}
\put(841,693){\makebox(0,0){$\times$}}
\put(854,699){\makebox(0,0){$\times$}}
\put(868,707){\makebox(0,0){$\times$}}
\put(881,706){\makebox(0,0){$\times$}}
\put(894,703){\makebox(0,0){$\times$}}
\put(907,715){\makebox(0,0){$\times$}}
\put(921,729){\makebox(0,0){$\times$}}
\put(934,717){\makebox(0,0){$\times$}}
\put(947,726){\makebox(0,0){$\times$}}
\put(961,730){\makebox(0,0){$\times$}}
\put(974,728){\makebox(0,0){$\times$}}
\put(987,742){\makebox(0,0){$\times$}}
\put(1000,740){\makebox(0,0){$\times$}}
\put(1014,740){\makebox(0,0){$\times$}}
\put(1027,741){\makebox(0,0){$\times$}}
\put(1040,753){\makebox(0,0){$\times$}}
\put(1054,750){\makebox(0,0){$\times$}}
\put(1067,745){\makebox(0,0){$\times$}}
\put(1080,750){\makebox(0,0){$\times$}}
\put(1093,758){\makebox(0,0){$\times$}}
\put(1107,761){\makebox(0,0){$\times$}}
\put(1120,760){\makebox(0,0){$\times$}}
\put(1133,760){\makebox(0,0){$\times$}}
\put(1147,768){\makebox(0,0){$\times$}}
\put(1160,770){\makebox(0,0){$\times$}}
\put(1173,762){\makebox(0,0){$\times$}}
\put(1186,765){\makebox(0,0){$\times$}}
\put(1200,773){\makebox(0,0){$\times$}}
\put(1213,785){\makebox(0,0){$\times$}}
\put(1226,788){\makebox(0,0){$\times$}}
\put(1240,773){\makebox(0,0){$\times$}}
\put(1253,782){\makebox(0,0){$\times$}}
\put(1266,776){\makebox(0,0){$\times$}}
\put(1280,775){\makebox(0,0){$\times$}}
\put(1293,775){\makebox(0,0){$\times$}}
\put(1306,785){\makebox(0,0){$\times$}}
\put(1319,780){\makebox(0,0){$\times$}}
\put(1333,782){\makebox(0,0){$\times$}}
\put(1346,800){\makebox(0,0){$\times$}}
\put(1359,804){\makebox(0,0){$\times$}}
\put(1373,803){\makebox(0,0){$\times$}}
\put(1386,794){\makebox(0,0){$\times$}}
\put(1399,797){\makebox(0,0){$\times$}}
\put(1412,797){\makebox(0,0){$\times$}}
\put(1426,796){\makebox(0,0){$\times$}}
\put(1349,777){\makebox(0,0){$\times$}}
\put(110.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(110.0,82.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{187.179pt}}
\put(110.0,859.0){\rule[-0.200pt]{320.156pt}{0.400pt}}
\end{picture}

